iSeg: Interactive 3D Segmentation via Interactive Attention

We present iSeg, a new interactive technique for segmenting 3D shapes. Previous works have focused mainly on leveraging pre-trained 2D foundation models for 3D segmentation based on text. However, text may be insufficient for accurately describing fine-grained spatial segmentations. Moreover, achieving a consistent 3D segmentation using a 2D model is highly challenging, since occluded areas of the same semantic region may not be visible together from any 2D view. Thus, we design a segmentation method conditioned on fine user clicks, which operates entirely in 3D. Our system accepts user clicks directly on the shape's surface, indicating the inclusion or exclusion of regions from the desired shape partition. To accommodate various click settings, we propose a novel interactive attention module capable of processing different numbers and types of clicks, enabling the training of a single unified interactive segmentation model. We apply iSeg to a myriad of shapes from different domains, demonstrating its versatility and faithfulness to the user's specifications. Our project page is at https://threedle.github.io/iSeg/.

==> figures/ablation/ablation_jpg.tex <==
\begin{figure}[!tbh]
\centering
\newcommand{\pl}{-4}
% trim: left, bottom, right, top
\begin{overpic}[width=0.99\linewidth, trim=0 0 0 -110, clip]
{figures/ablation/ablation.jpg}
\put(1,  \pl){\textcolor{black}{Ablation (train)}}
\put(29,  \pl){\textcolor{black}{Ours (train)}}
\put(56,  \pl){\textcolor{black}{Ablation (test)}}
\put(82,  \pl){\textcolor{black}{Ours (test)}}
\end{overpic}
\vspace{2mm}
\captionof{figure}{\textbf{Ablation test.} We compare an \ourmethod{} model from separate training of the encoder and decoder with an ablation model from joint training of both components. Our proposed separate training scheme results in better generalization for test vertices.}
\label{fig:ablation}
\end{figure}


==> figures/cross/cross_png.tex <==
\begin{figure}
\centering
\newcommand{\pl}{-2}
% trim: left, bottom, right, top
\begin{overpic}[width=\linewidth, trim=300 50 170 0, clip]{figures/cross/cross.png}
\put(1,  \pl){\textcolor{black}{Clicked point}}
\put(27,  \pl){\textcolor{black}{Self-segmentation}}
\put(63,  \pl){\textcolor{black}{Cross-segmentation}}
\put(19.5,  82){\textcolor{black}{Human}}
\put(19,  77.5){\textcolor{black}{decoder}}
\put(19.5,  16.5){\textcolor{black}{Human}}
\put(19,  12){\textcolor{black}{decoder}}
\put(50,  87.5){\textcolor{black}{Horse decoder}}
\put(51.5,  33){\textcolor{black}{Airplane}}
\put(52,  28.5){\textcolor{black}{decoder}}
\end{overpic}
\vspace{-3mm}
\captionof{figure}{\textbf{Cross-domain segmentation.} \ourmethod{} optimizes a condition-agnostic feature field, which is capable of transferring between shapes. The feature vector of a point click of one mesh (left) is used to segment the same shape (middle) as well as \textit{another} shape from a \textit{different} domain (right).}
\label{fig:cross_seg}
\end{figure}


==> figures/edits/edits_png.tex <==
\begin{figure*}[tb!]
\centering
\newcommand{\pl}{1}
% trim: left, bottom, right, top
\begin{overpic}[width=\linewidth, trim=220 200 310 0, clip]{figures/edits/edits_supp.png}
\put(18,  \pl){\textcolor{black}{\small{Delete}}}
\put(45,  \pl){\textcolor{black}{\small{Select}}}
\put(67,  \pl){\textcolor{black}{\small{Shrink}}}
\put(93,  \pl){\textcolor{black}{\small{Extrude}}}
\end{overpic}
\captionof{figure}{\textbf{Local geometric edits.} Our localized and contiguous segmentations enable various shape edits, such as deleting or selecting the segmented region, shrinking it, or extruding it along the surface normal.}
\label{fig:edits_supp}
\end{figure*}


==> figures/effectiveness/effectiveness_png.tex <==
\begin{figure*}
\begin{center}
    \centering
    \newcommand{\pl}{-2}
    % trim: left, bottom, right, top
    \begin{overpic}[width=\textwidth, trim=0 0 0 0, clip]{figures/effectiveness/effectiveness.png}
    \put(37, 26){\textcolor{black}{Completely effective segmentation}}
    \put(39, 12){\textcolor{black}{Partially effective segmentation}}
    \put(37, -2){\textcolor{black}{Completely ineffective segmentation}}
    \end{overpic}
    \vspace{0.5mm}
    \captionof{figure}{\textbf{Segmentation effectiveness.} We visualize results with a varying level of effectiveness, as presented in our perceptual user study. The segmentations from top to bottom rows are considered completely effective, partially effective, and completely ineffective, respectively.}
    \label{fig:effectiveness}
\end{center}
\end{figure*}


==> figures/limitation/limitation_png.tex <==
\begin{figure}[!t]
\centering
\newcommand{\pl}{-2}
% trim: left, bottom, right, top
\begin{overpic}[width=0.8\linewidth, trim=30 50 30 100, clip]{figures/limitation/limitation.png}
\put(10,  \pl){\textcolor{black}{First view}}
\put(68,  \pl){\textcolor{black}{Second view}}
\end{overpic}
% \vspace{-3mm}
\captionof{figure}{\textbf{Limitation.} \ourmethod{} may not produce a symmetric segmentation result for a symmetric shape. In this case, the segmented region of one side of the shape is different than the other.}
\label{fig:limitation}
\end{figure}


==> figures/occluded/occluded_png.tex <==
\begin{figure}[!tbh]
\begin{center}
\centering
\newcommand{\pl}{-3}
% trim: left, bottom, right, top
\begin{overpic}[width=0.99\linewidth, trim=0 0 0 0, clip]
{figures/occluded/occluded.png}
\put(49.5, 41){\textcolor[rgb]{0.24,0.83,0.24}{Click}}
\put(90, 41){\textcolor[rgb]{0.24,0.83,0.24}{Click}}
\put(32, \pl){\textcolor{black}{\ourmethod{} (ours)}}
\put(72, \pl){\textcolor{black}{SAM Baseline}}
\end{overpic}
\caption{\textbf{The power of \ourmethod{} for occluded point click.} When the point click (green dot in the leftmost image) is occluded, \ourmethod{} can produce an effective 3D segmentation (highlighted in blue), whereas the SAM baseline is unable to do so.}
\label{fig:sam_occlude}
\end{center}
\end{figure}


==> figures/partnet/partnet_png.tex <==
\begin{figure}[!t]
\centering
\newcommand{\pl}{-0.5}
% trim: left, bottom, right, top
\begin{overpic}[width=\linewidth, trim=0 50 0 100, clip]{figures/partnet/partnet.png}
\put(1.5,  \pl){\textcolor{black}{InterObject3D}}
\put(27, \pl){\textcolor{black}{SAM Baseline}}
\put(54.5, \pl){\textcolor{black}{iSeg (ours)}}
\put(77.8, \pl){\textcolor{black}{Ground-truth}}
\end{overpic}
\vspace{-5mm}
\caption{\siga{\textbf{Segmentation comparison on PartNet.} Each pair shows different views of the segmentation result for different interactive techniques. The other methods produce a partial segmentation of the part containing the click. In contrast, \ourmethod{} obtains an accurate result, which is similar to the ground-truth annotation of the part.}}
\label{fig:partnet}
\end{figure}


==> figures/sequential/sequential_png.tex <==
\begin{figure}[!t]
\centering
\newcommand{\pl}{-2}
% trim: left, bottom, right, top
%\vspace{-2pt}
\begin{overpic}[width=0.99\linewidth, trim=0 0 0 -44.5]{figures/sequential/sequential.png}
\put(12,  \pl){\textcolor{black}{First positive}}
\put(43,  \pl){\textcolor{black}{Second negative}}
\put(77,  \pl){\textcolor{black}{Third positive}}
\end{overpic}
%\vspace{-2mm}
\captionof{figure}{\textbf{Customized segmentations.} \ourmethod{} is capable of creating customized segmentations specified by several input clicks.}
\label{fig:sequential_seg}
\end{figure}


==> figures/teaser/teaser_png.tex <==
\begin{teaserfigure}
\begin{center}
    \centering
    \newcommand{\pl}{-2}
    % trim: left, bottom, right, top
    \begin{overpic}[width=\textwidth, trim=10 200 20 200, clip]{figures/teaser/teaser.png}
    \put(8.5,  \pl){\textcolor{black}{Single positive click}}
    \put(31.5,  \pl){\textcolor{black}{Second positive click}}
    \put(59,  \pl){\textcolor{black}{Single positive click}}
    \put(82,  \pl){\textcolor{black}{Second negative click}}
    \end{overpic}
    \vspace{-2mm}
    \captionof{figure}{\ourmethod{} computes customized fine-grained segmentations on shapes interactively specified by user clicks. The clicks, denoted by a green or a red dot, indicate whether to include or exclude regions, respectively. Our method is capable of segmenting regions that are not accurately specified by text.}
    \label{fig:teaser}
\end{center}
\end{teaserfigure}


==> figures/view_generalization/view_generalization_png.tex <==
\begin{figure}
\centering
\newcommand{\pl}{-2}
% trim: left, bottom, right, top
\begin{overpic}[width=\linewidth, trim=230 60 260 20, clip]{figures/view_generalization/view_generalization.png}
\put(12,  \pl){\textcolor{black}{Single positive click}}
\put(61,  \pl){\textcolor{black}{Two positive clicks}}
\end{overpic}
\vspace{-2mm}
\captionof{figure}{\textbf{Native 3D segmentation.} \ourmethod{} segments parts in a 3D-consistent manner, regardless of whether the surface is occluded from the point click. A point is selected on the back of the chair (left), which is not visible from the front view. Still, our method delineates the occluded surface even though the 2D training data cannot contain this information. Furthermore, we may input two point clicks occluded from each other, one on the back of the chair and one on the front (right). These points cannot be simultaneously input to any 2D decoder, as they are not visible concurrently from any single viewpoint. Nonetheless, \ourmethod{} faithfully segments the whole backrest part.}
\label{fig:view_generalization}
\end{figure}

